RIGID: Recurrent GAN Inversion and Editing of Real Face Videos

GAN inversion is indispensable for applying the powerful editability of GAN to real images. However, existing methods invert video frames individually often leading to undesired inconsistent results over time. In this paper, we propose a unified recurrent framework, named \textbf{R}ecurrent v\textbf{I}deo \textbf{G}AN \textbf{I}nversion and e\textbf{D}iting (RIGID), to explicitly and simultaneously enforce temporally coherent GAN inversion and facial editing of real videos. Our approach models the temporal relations between current and previous frames from three aspects. To enable a faithful real video reconstruction, we first maximize the inversion fidelity and consistency by learning a temporal compensated latent code. Second, we observe incoherent noises lie in the high-frequency domain that can be disentangled from the latent space. Third, to remove the inconsistency after attribute manipulation, we propose an \textit{in-between frame composition constraint} such that the arbitrary frame must be a direct composite of its neighboring frames. Our unified framework learns the inherent coherence between input frames in an end-to-end manner, and therefore it is agnostic to a specific attribute and can be applied to arbitrary editing of the same video without re-training. Extensive experiments demonstrate that RIGID outperforms state-of-the-art methods qualitatively and quantitatively in both inversion and editing tasks. The deliverables can be found in \url{https://cnnlstm.github.io/RIGID}

==> edit_ablation.tex <==
\begin{figure}[t]
    \flushleft
    % \centering
    \captionsetup[subfloat]{labelformat=empty,justification=centering}
    \subfloat[]{
    \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0005}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0005}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0005}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0005}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0005}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0005}
     \end{minipage}
     }
   \hspace{-2.8mm}
   \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0010}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0010}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0010}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0010}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0010}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0010}
     \end{minipage}
     }
   \hspace{-2.8mm}
   \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0021}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0021}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0021}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0021}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0021}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0021}
     \end{minipage}
     }
   \hspace{-2.8mm}
    \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0047}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0047}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0047}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0047}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0047}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0047}
    \end{minipage}
     }
    \hspace{-2.8mm}
    \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0057}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0057}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0057}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0057}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0057}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0057}
    \end{minipage}
     }
    \hspace{-2.8mm}
    \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0075}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0075}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0075}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0075}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0075}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0075}
    \end{minipage}
     }
    \hspace{-2.8mm}
    \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0086}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0086}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0086}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0086}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0086}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0086}
    \end{minipage}
     }
    \hspace{-2.8mm}
    \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0096}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0096}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0096}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0096}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0096}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0096}
    \end{minipage}
     }
    \hspace{-2.8mm}
    \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0108}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0108}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0108}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0108}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0108}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0108}
    \end{minipage}
     }    
    \hspace{-2.8mm}
    \subfloat[]{
     \begin{minipage}{0.095\linewidth}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/ORI/01-02-02-02-01-01-10/frame0118}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/LT/01-02-02-02-01-01-10_Male_rep/frame0118}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_Noise_32/01-02-02-02-01-01-10_Male_rep/frame0118}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_LCSS_32/01-02-02-02-01-01-10_Male_rep/frame0118}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/WO_IFSC_32/01-02-02-02-01-01-10_Male_rep/frame0118}
     \includegraphics[width=\linewidth]{figure/edit/RAVDESS/FULL_32/01-02-02-02-01-01-10_Male_rep/frame0118}
    \end{minipage}
     }
\rotatebox[origin=c]{270}{\hspace{1mm} \tiny{Ori.} \hspace{5mm} \tiny{BaseL.} \hspace{5mm} \tiny{$w/o$ N.M.} \hspace{3mm} \tiny{$w/o$ LCSS}  \hspace{3mm} \tiny{$w/o$ $\mathcal{L}_{ifsc}$} \hspace{5mm} \tiny{Ours} }
\caption{Qualitative comparison of various variants on video editing.}
\label{fig:ablation_exp}\vspace{-4mm}
\end{figure}


==> supp_1.tex <==
\begin{figure*}
    \centering
    \subfloat[\footnotesize{Original}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/edit/IN_THE_WILD_CROP/ORI/jim/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/edit/IN_THE_WILD_CROP/ORI/jim/}{0100}{0148}%\\
    \end{minipage}
    }
    \hspace{-2.25mm}
    \subfloat[\footnotesize{IGCI}\label{fig_igci}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/rec/IN_THE_WILD_CROP/XU/jim/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/edit/IN_THE_WILD_CROP/XU/jim_Chubby_rep/}{0100}{0148}%\\
    \end{minipage}
    }
    \hspace{-2.25mm}
    \subfloat[\footnotesize{Latent-T}\label{fig_lt}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/rec/IN_THE_WILD_CROP/Latent_T/jim/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/edit/IN_THE_WILD_CROP/LT/jim_Chubby_rep/}{0100}{0148}%\\
    \end{minipage}
    }
    \hspace{-2.25mm}
    \subfloat[\footnotesize{STIT}\label{fig_stit}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/rec/IN_THE_WILD_CROP/STIT/jim/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/edit/IN_THE_WILD_CROP/STIT/jim_Chubby_rep/}{0100}{0148}%\\
    \end{minipage}
    }
    \hspace{-2.25mm}
    \subfloat[\footnotesize{RIGID}\label{fig_rigid}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/rec/IN_THE_WILD_CROP/FULL_32/jim/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{24}{figure/edit/IN_THE_WILD_CROP/FULL_32/jim_Chubby_rep/}{0100}{0148}%\\
    \end{minipage}
    }
    \rotatebox[origin=c]{270}{ \small{\texttt{+Chubby}} \hspace{-45mm} \small{\texttt{Inversion}}}\\
    % \rotatebox[origin=c]{270}{\hspace{-60mm} \small{\texttt{+Chubby}} \hspace{-50mm} \small{\texttt{Inversion}}}\\


\caption{Comparisons of video inversion and editing with existing methods. Our RIGID achieves temporal coherent inversion and editing performances. IGIC and Latent-Transformer cannot provide consistent results both for inversion and editing. STIT cannot support the ``Chubby'' editing. This figure contains \emph{animated videos}, which are best viewed using Adobe Acrobat.}
\label{fig:qualitative}
% \vspace{-0.75cm}
\end{figure*}


==> teaser_bbb.tex <==
\begin{figure}
    \centering
    \subfloat[\footnotesize{Original}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_ori/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_ori/}{0100}{0148}
    \end{minipage}
    }
    \hspace{-2.25mm}
    \subfloat[\footnotesize{IGCI / 120,000s}\label{fig_igci}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_rec_xu/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_Chubby_xu/}{0100}{0148}
    \end{minipage}
    }
    \hspace{-2.25mm}
    \subfloat[\footnotesize{Latent-T. / 49.2s}\label{fig_lt}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_rec_lt/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_Chubby_lt/}{0100}{0148}
    \end{minipage}
    }
    \hspace{-2.25mm}
    \subfloat[\footnotesize{STIT / 1,600s}\label{fig_stit}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_rec_stit/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_Chubby_stit/}{0100}{0148}
    \end{minipage}
    }
    \hspace{-2.25mm}
    \subfloat[\footnotesize{RIGID / 54.5s}\label{fig_rigid}]{
    \begin{minipage}{0.19\linewidth}
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_rec_ours/}{0100}{0148}\\
    \animategraphics[autoplay,loop,width=\textwidth]{15}{figure/teaser_bb/bb_Chubby_ours/}{0100}{0148}
    \end{minipage}
    }
    \rotatebox[origin=c]{270}{ \small{\texttt{+Chubby}} \hspace{-45mm} \small{\texttt{Inversion}}}\\
\caption{Comparisons of video inversion and editing with existing methods. Number in each column denotes the average editing time over 100 frames. Our RIGID achieves temporal coherent inversion and editing performances with much less time cost. This figure contains \emph{animated videos}, which are best viewed using Adobe Acrobat.}
\label{fig:teaser}
% \vspace{-0.75cm}
\end{figure}

